Studying Image Diffusion Features for Zero-Shot Video Object Segmentation

This paper investigates the use of large-scale diffusion models for Zero-Shot Video Object Segmentation (ZS-VOS) without fine-tuning on video data or training on any image segmentation data. While diffusion models have demonstrated strong visual representations across various tasks, their direct application to ZS-VOS remains underexplored. Our goal is to find the optimal feature extraction process for ZS-VOS by identifying the most suitable time step and layer from which to extract features. We further analyze the affinity of these features and observe a strong correlation with point correspondences. Through extensive experiments on DAVIS-17 and MOSE, we find that diffusion models trained on ImageNet outperform those trained on larger, more diverse datasets for ZS-VOS. Additionally, we highlight the importance of point correspondences in achieving high segmentation accuracy, and we yield state-of-the-art results in ZS-VOS. Finally, our approach performs on par with models trained on expensive image segmentation datasets.

==> tab/fitlter_corrs_backup.tex <==
\footnotesize
\centering
\begin{NiceTabular}
{lc@{\hspace{10pt}}C{4.2em}@{}C{4.2em}@{}C{4.2em}}[colortbl-like]
\toprule
& & \multicolumn{3}{c}{\small DAVIS-17 val} \\
\cmidrule(lr){3-5} 
Model  & Filtering &  \mjf & \mj & \mf \\
\midrule
\multirow{3}{*}{SD-1.2} & None & 69.9 &67.3  &72.6   \\
&Heuristic & \underline{70.3}\textsubscript{\color{ourgreen}$\blacktriangle $0.4}&\underline{67.5}\textsubscript{\color{ourgreen}$\blacktriangle $0.2} &\underline{73.1}\textsubscript{\color{ourgreen}$\blacktriangle $0.5}  \\ 
&Oracle &   &    &    \\
\hdashline
\multirow{3}{*}{SD-1.3} & None & 69.2 & 66.5 & 72.0  \\
&Heuristic & \underline{69.5}\textsubscript{\color{ourgreen}$\blacktriangle $0.3} & \underline{66.6}\textsubscript{\color{ourgreen}$\blacktriangle $0.1}   & \underline{72.4}\textsubscript{\color{ourgreen}$\blacktriangle $0.4}\\ 
&Oracle &   &    &    \\ 
\hdashline
\multirow{3}{*}{SD-1.4} & None & 68.9 & 66.0  & 71.8 \\
&Heuristic & \underline{69.2}\textsubscript{\color{ourgreen}$\blacktriangle $0.3} & \underline{66.1}\textsubscript{\color{ourgreen}$\blacktriangle $0.1}   & \underline{72.1}\textsubscript{\color{ourgreen}$\blacktriangle $0.5}    \\
&Oracle &   &    &    \\ 
\hdashline
\multirow{3}{*}{SD-1.5} & None & 68.8 & 66.0 &  71.6 \\
&Heuristic &  \underline{69.3}\textsubscript{\color{ourgreen}$\blacktriangle $0.5} & \underline{66.5}\textsubscript{\color{ourgreen}$\blacktriangle $0.5} &  \underline{72.1}\textsubscript{\color{ourgreen}$\blacktriangle $0.5}   \\
& Oracle &   &    &    \\ 
\hdashline
\multirow{3}{*}{SD-2.1} & None & 69.8 & 67.1 & 72.6 \\
& Heuristic & \underline{70.2}\textsubscript{\color{ourgreen}$\blacktriangle $0.4} & \underline{67.2}\textsubscript{\color{ourgreen}$\blacktriangle $0.1} & \underline{73.1}\textsubscript{\color{ourgreen}$\blacktriangle $0.5} \\
& Oracle &  \textbf{83.3}\textsubscript{\color{ourgreen}$\blacktriangle $13.5} &  \textbf{77.8}\textsubscript{\color{ourgreen}$\blacktriangle $10.7} &  \textbf{88.9}\textsubscript{\color{ourgreen}$\blacktriangle $16.3} \\ 
\hdashline
\multirow{3}{*}{ADM} & None &  76.1 &73.2  & 79.1  \\
&Heuristic &  \underline{76.8}\textsubscript{\color{ourgreen}$\blacktriangle $0.7} & \underline{73.8} \textsubscript{\color{ourgreen}$\blacktriangle $0.6}   &  \underline{79.7}\textsubscript{\color{ourgreen}$\blacktriangle $0.7}  \\ 
&Oracle &   &    &    \\ 
\bottomrule
\end{NiceTabular}
% 

==> tab/tab1.tex <==
\footnotesize
\centering
\begin{NiceTabular}
{lc@{\hspace{10pt}}C{2.2em}@{}C{2.2em}@{}C{2.2em}}[colortbl-like]
\toprule
& & \multicolumn{3}{c}{\small DAVIS-17 val} \\
\cmidrule(lr){3-5} 
Model  & Text&  \mjf & \mj & \mf \\
\bottomrule
ResNet18  &-  &30.9 & & \\
ResNet50 & - &32.6 & & \\
ResNet101  & - &34.6 & & \\
DinoV2   & - &71.4 & & \\
\toprule
\multicolumn{6}{l}{\textbf{\textit{Text-analysis}}} \\
\midrule
SD 2.1 & - & 69.8 & & \\
SD 2.1 & random &  & & \\
SD 2.1 & ground-truth & 70.2 &67.3 &73.1 \\
\toprule
\multicolumn{6}{l}{\textbf{\textit{Textual inversion}}} \\
\midrule
SD 2.1 & - &  & & \\
\toprule
\multicolumn{6}{l}{\textbf{\textit{Drop FG-BG correspondences}}} \\
\midrule
SD 2.1 & - &83.3&77.8 &88.9 \\
\bottomrule
\end{NiceTabular}
% 
